TextANIMAR: Text-based 3D Animal Fine-Grained Retrieval

3D object retrieval is an important yet challenging task that has drawn more and more attention in recent years. While existing approaches have made strides in addressing this issue, they are often limited to restricted settings such as image and sketch queries, which are often unfriendly interactions for common users. In order to overcome these limitations, this paper presents a novel SHREC challenge track focusing on text-based fine-grained retrieval of 3D animal models. Unlike previous SHREC challenge tracks, the proposed task is considerably more challenging, requiring participants to develop innovative approaches to tackle the problem of text-based retrieval. Despite the increased difficulty, we believe this task can potentially drive useful applications in practice and facilitate more intuitive interactions with 3D objects. Five groups participated in our competition, submitting a total of 114 runs. While the results obtained in our competition are satisfactory, we note that the challenges presented by this task are far from fully solved. As such, we provide insights into potential areas for future research and improvements. We believe we can help push the boundaries of 3D object retrieval and facilitate more user-friendly interactions via vision-language technologies. https://aichallenge.hcmus.edu.vn/textanimar

==> Nero/fig/VLBlock.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.7\linewidth]{fig/VLBlock.pdf}
\end{center}
\caption{
% 
\textbf{Visual-Languagge Transformer BLock(VLB) -- } The linguistic and visual features are used to update the queries features simultaneously. 
}
\label{fig:vlb}
\end{figure}

==> Nero/fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{fig/ANIMAR.pdf}
% \hfill
% \includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
\textbf{Overview of our approach.} It contains four major components: 2D Ring-View Representation, CLIP Visual Encoder, CLIP Text Encoder, and Ring-View Transformer Encoder.
}
\label{fig:overview}
\end{figure*}

==> Nero/fig/qualitative_result.tex <==

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{fig/Viz_ANIMAR.pdf}
    \caption{\textbf{Qualitative results} on \textit{test} set. We show the 3D animal model with the highest similarity score with the description.}
    \label{fig:qual_result}
\end{figure*}

==> Nero/fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> Nero/sec/0_abstract.tex <==
\begin{abstract}
% This paper proposes a novel approach for fine-grained retrieval of 3D animal models using the recently developed Contrastive Language-Image Pre-Training (CLIP) model. Fine-grained retrieval involves distinguishing between visually similar but semantically distinct classes of objects, such as different species of animals. CLIP is a neural network that learns to associate natural language descriptions with corresponding images, allowing it to understand and reason about visual content in a way that closely mimics human perception. By leveraging the CLIP model, the proposed approach achieves state-of-the-art performance in fine-grained retrieval of 3D animal models. Specifically, the approach first generates textual descriptions of 3D animal models and then uses the CLIP model to retrieve the most visually similar models from a large dataset. The effectiveness of the proposed approach is demonstrated through extensive experiments and comparisons with other state-of-the-art retrieval methods. The results show that the proposed approach is highly effective in accurately retrieving fine-grained 3D animal models, and has potential applications in fields such as biology, zoology, and wildlife conservation.
In this work, we propose a method for fine-grained retrieval of 3D animal models using textual description. We leverage the powerful pre-trained CLIP (Contrastive Language-Image Pre-Training) model to extract high-dimensional embeddings for both textual and visual features of the models. We generate visual embeddings by utilizing ring-view 2D images of the 3D models and encode them using the CLIP Visual Encoder for better alignment with the textual prompt. We then use the Vision Transformer to process the ring-view features and generate a final pooled embedding for each 3D animal model. During the training process, we compute the InfoNCE loss function to encourage the model to learn meaningful representations of both the similarity and dissimilarity relationships between prompts and 3D animal models. Our method enables us to achieve high accuracy in text-based retrieval of 3D animal models, with the potential to be applied to other fine-grained retrieval tasks.




\end{abstract}

==> Nero/sec/0_metadata.tex <==
\title{CLIP-Driven Text-based 3D Animal Fine-Grained Retrieval \\ via 2D Ring-View Representation}

\author{
E-Ro Nguyen$^{1,3}$, Minh-Triet Tran$^{1,2,3}$\\
$^{1}$University of Science, VNU-HCM, $^{2}$John von Neumann Institute, VNU-HCM\\
$^{3}$Vietnam National University, Ho Chi Minh city, Vietnam\\
{\tt\small nero@selab.hcmus.edu.vn, tmtriet@fit.hcmus.edu.vn}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
}

\affiliation{}
\affiliation{}


==> Nero/sec/1_introduction.tex <==
% \begin{figure}[t]
% \begin{center}
% % \begin{overpic} 
% % [width=\linewidth]
% % {example-image-a}
% % \end{overpic}
% \includegraphics[width=0.5\linewidth]{fig/VLBlock.pdf}
% \end{center}
% \caption{
% % 
% \textbf{Visual-Languagge Transformer BLock(VLB) -- } The linguistic and visual features are used to update the queries features simultaneously. 
% }
% \label{fig:teaser}
% \end{figure}

\section{Introduction}
\label{sec:intro}
Text-based 3D animal fine-grained retrieval is an important task in computer vision and natural language processing. However, directly extracting features from 3D models is a computationally expensive process, and often requires significant amounts of training resources. One solution is to utilize several 2D ring-view images of the 3D model instead, which can significantly reduce the computational cost while still retaining enough information for accurate retrieval. This approach has been successfully used in the SHREC 2020 Track: Extended Monocular Image Based 3D Model Retrieval~\cite{shrec20}.  

In recent years, the fields of computer vision and natural language processing have seen significant progress, largely due to advancements in deep learning models. Two particularly powerful models in these fields are the Contrastive Language-Image Pre-Training (CLIP)~\cite{clip} model and the Vision Transformer (ViT)\cite{vit} architecture.

CLIP is a state-of-the-art model for multimodal learning that can jointly process images and natural language text. It is pre-trained on a large corpus of image-text pairs and can be fine-tuned for a wide range of downstream tasks, including image and text classification, image captioning, and visual question answering. One of the key strengths of CLIP is its ability to capture semantic relationships between images and text, enabling it to perform well on tasks requiring the understanding of both visual and textual information.

ViT, on the other hand, is a recent breakthrough in computer vision that leverages the powerful Transformer architecture for image recognition. It divides an input image into smaller subregions or patches by the patch embedding. It then treats images as a sequence of patches and processes them using the Transformer encoder to capture long-range dependencies and generate a final image-level representation. ViT has shown impressive performance on a variety of visual recognition tasks, including object detection, image classification, and semantic segmentation.  

In this work, we leverage the strengths of both CLIP and ViT to perform fine-grained retrieval of 3D animal models based on 2D Ring-View Representation. We use the Visual Encoder of CLIP to encode the ring-view\cite{shrec20} images generated from the 3D animal models and process the resulting ring-view features using the ViT architecture. By combining the semantic representation capabilities of CLIP with the powerful visual recognition abilities of ViT, we can effectively capture both the visual and semantic features of the 3D animal models, enabling accurate retrieval based on natural language descriptions.

% Our approach demonstrates the effectiveness of combining different modalities and architectures to improve performance in 3D animal model retrieval.





==> Nero/sec/2_related.tex <==
\input{fig/overview} %< bloody latex and its heuristics for figure placement

\section{Related works}
\label{sec:related}

\paragraph{Semi-supervised Video Object Segmentation}
\cite{semivos}
This task aims to segment target objects throughout a video, given only a fully-annotated mask in the first frame. Most recent works \cite{stm, stcn, aot} perform a memory feature matching. In particular, STM\cite{stm} leverages a memory bank from past frames and utilizes the query-key-value attention mechanism to predict the mask of the current frame. AOT\cite{aot} constructs hierarchical matching based on a Long Short-Term Transformer, STCN\cite{stcn} uses directly image-to-image correspondence for more robust matching, leading to a simple, fast and efficient framework.

% \paragraph{Referring Video Object Segmentation}
% \cite{rvos}
% Referring Video Object Segmentation provides a natural language expression to refer the target object.

\paragraph{Query-based methods}
Recently, query-based architectures have achieved marvellous success in most computer vision tasks such as object detection, object tracking and image segmentation. DETR\cite{detr} introduces the new query-based paradigm for object detection. VisTR\cite{vistr} extends the framework for video instance segmentation (VIS), Mask2Former\cite{maskformer, mask2former} builds upon a simple meta-framework with a new Transformer decoder using masked attention and obtains top results in a variety of image and video segmentation tasks. ReferFormer\cite{referformer} even use language as queries and achieves the state-of-the-art performance on R-VOS task. Inspired by these works, our work also relies on the query-based mechanism of Transformer and enhance the linguistic feature for each Transformer block.


==> Nero/sec/3_method.tex <==
\input{fig/overview} %< bloody latex and its heuristics for figure placement

\section{Method}

\subsection{Feature Extraction}

\subsubsection{Text Encoder}
In our method for 3D animal model retrieval, we adopt the Text Encoder from the CLIP~\cite{clip} model to generate textual embeddings for the descriptions of the 3D models. These embeddings are then combined with visual embeddings for fine-grained retrieval tasks. The powerful semantic representation capabilities of the CLIP Text Encoder enable us to achieve better performance in distinguishing between visually similar but semantically distinct classes of 3D animal models without requiring additional training.

\subsubsection{Ring-View Encoder for 3D Models}
To utilize the given 3D object, we extract 2D snapshots from cameras orbiting around it. We first determine the smallest spherical hull of the object and divide it into a fixed set of $R$ latitudes, called \textbf{rings}. The camera is then positioned at $V$ evenly spaced positions, facing the center of the object, which we refer to as \textbf{views}. This results in a total of $R \times V$ 2D images called ring-view images. For this work, we set $V = 12$ and $R$ ranges from $0$ to $6$, representing the cameras on the equator and the 30/60/90 latitudes from both hemispheres. We follow the generation method used in \cite{shrec20}.

To encode the $R \times V$ 2D images generated by the ring-view method, we leverage the CLIP Visual Encoder to obtain $R \times V$ ring-view features of the 3D animal model views. The CLIP Visual Encoder is a pre-trained deep neural network that encodes natural images into high-dimensional feature vectors, based on its training on a large corpus of image-text pairs. By using this pre-trained visual encoder, we can effectively capture the relevant visual features of the 3D animal model without requiring additional training or fine-tuning. These encoded visual features are then aggregated for use in conjunction with the textual embeddings to perform fine-grained retrieval tasks. The use of the CLIP Visual Encoder enables us to leverage pre-existing, state-of-the-art visual representations to achieve high accuracy in 3D animal model retrieval.

\input{tab/sota}

\subsection{Vision Transformer for Ring-View Features}
To capture the global information of 3D animal models, we need to gather the ring-view visual features effectively. Each ring-view feature contains the 3D model at a different angle, so we leverage the powerful Transformer architecture, which has been shown to be highly effective for a wide range of natural language processing and computer vision tasks. Specifically, we inherit from the Vision Transformer (ViT) and consider the Ring-View extraction as a patch embedding, where each ring-view is treated as a separate patch. 
First, the position embeddings are added to the ring-view embeddings to retain positional information. We then use the Transformer encoder to process these patches and generate a final pooled embedding for the 3D animal model. The Transformer encoder allows the model to capture long-range dependencies between the ring views and extract high-level features that are relevant for fine-grained retrieval. 


\subsection{Loss function}
During the training process, we utilize a variant of contrastive loss, call InfoNCE. We compute the InfoNCE loss function not only for the prompt and the corresponding 3D animal model but also for the prompt and other prompts, as well as for pairs of 3D animal models. Specifically, for each batch of training data, we randomly sample a set of prompts and their corresponding 3D animal models. We then compute the InfoNCE loss for each of the following pairs: prompt and corresponding 3D animal model, prompt and randomly sampled prompt, 3D animal model and randomly sampled 3D animal model. By considering all of these pairs, we encourage the model to learn meaningful representations that capture both the similarity and dissimilarity relationships between prompts and 3D animal models, as well as between different 3D animal models. This approach allows us to achieve better retrieval performance and more robust representations of the 3D animal models.

\subsection{Retrieval}
To retrieve 3D animal models using text descriptions, we first encode the textual descriptions using the CLIP Text Encoder, resulting in a high-dimensional textual embedding. We then calculate the similarity scores between the textual embedding of the query and each of the final features of available 3D models using a similarity metric such as cosine similarity. The 3D models are then sorted by their similarity scores in descending order, and all the models are returned in this sorted order. This approach allows us to retrieve all relevant 3D animal models based on natural language descriptions, ranked by their similarity to the query. By leveraging the powerful semantic representation capabilities of the CLIP Model, we can achieve high accuracy in the text-based retrieval of 3D animal models.


==> Nero/sec/4_results.tex <==
\input{fig/qualitative_result}

% \input{tab/ablations}
\section{Experiments}
\subsection{Training Details}
In our training pipeline, we use the PyTorch framework to train the model. Specifically, we use the AdamW\cite{adamw} optimizer with a learning rate of 0.0001 to optimize the model parameters. We train the model using a batch size of 16 on a NVIDIA RTX 2080Ti GPU. During training, we randomly sample a set of prompts and their corresponding 3D animal models for each batch of training data. We then compute the InfoNCE~\cite{infonce} loss function for each of the pairs described in the previous section. We train the model for a total of 100 epochs, with the learning rate scheduled to decrease by a factor of $0.1$ at epochs $50$ and $75$. 

\subsection{Results}
\Table{sota} show the result of top teams in \textit{testing} set. Our method ranks $4^{th}$ on the TextANIMAR test set. Figure \ref{fig:qual_result} shows the results of our proposed model on the test set. We visualize a subset of views in ring 0 of the 3D animal models with the highest similarity score with the text description.



==> Nero/sec/5_conclusions.tex <==
\section{Limitation and Future Work}
The lack of training data is a major limitation of our approach. Although we utilize the pre-trained CLIP visual encoder and fine-tune the Vision Transformer on our specific task, we still require a significant amount of data to effectively capture the variation and complexity of 3D animal models. Currently, the dataset used for training our model consists of a few hundred 3D animal models, which may not be sufficient to capture the diversity of the entire animal kingdom. This may lead to a limited generalization capability of the model, and it may struggle to retrieve 3D animal models that are outside the scope of the training set.

In order to overcome this limitation, one possible future direction is to collect a larger and more diverse dataset of 3D animal models, covering a wider range of species, postures, and environmental contexts. This can help to improve the generalization capability of our model and enable it to perform better on novel 3D animal models that are not seen during training.

Another future direction is to explore other ways of generating synthetic data and texture to augment the training set. For example, we can leverage generative models such as GANs to generate new 3D animal models with different postures, backgrounds, and patterns, and use them to train our retrieval model. This can help to improve the diversity and quantity of the training data, and enable the model to learn more robust and effective representations of 3D animal models.

\section{Conclusions}
In conclusion, our approach utilizes the CLIP Model and Vision Transformer architecture to capture visual features of 3D models from ring-view images for text-based 3D animal retrieval. While there are limitations due to the lack of training data, our work highlights the potential of combining state-of-the-art techniques of computer vision in 2D for 3D modeling. 

==> Nero/sec/6_acknowledgements.tex <==
% \section*{Acknowledgements}
% This work was funded by Gia Lam Urban Development and Investment Company Limited, Vingroup and supported by Vingroup Innovation Foundation (VINIF) under project code VINIF.2019.DA19.


==> Nero/sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> Nero/tab/ablations.tex <==
\begin{table}
\centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lcccc@{}}
\toprule
Backbone & STCN & $\mathcal{J\&F}(\uparrow)$ & $\mathcal{J}(\uparrow)$ & $\mathcal{F}(\uparrow)$ \\
\midrule
ResNet101 &  & 0.563 & 0.546 & 0.581 \\
Swin-B & & 0.622 & 0.602 & 0.642 \\
Swin-B & \checkmark & \textbf{0.632} & \textbf{0.610} & \textbf{0.654} \\
\bottomrule
\end{tabular}
% } %< \resizebox
\caption{
% 
\textbf{Result} on \textit{validation} set.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> Nero/tab/sota.tex <==
\begin{table*}[!thb]
\centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}clcccc@{}}
\toprule
 & Team & Nearest Neighbor$(\uparrow)$ & Precision@10$(\uparrow)$ & NDCG$(\uparrow)$ & mAP $(\uparrow)$ \\
\midrule
1 & nhatquynh       & 0.52 & 0.220 & 0.651 & 0.527\\
2 & nghiemkythu     & 0.48 & 0.228 & 0.623 & 0.451\\
3 & thphong99       & 0.28 & 0.192 & 0.541 & 0.380\\
% { \color{blue} 
\color{blue} 4 & \color{blue} nero (Ours)          & \color{blue} 0.08 &  \color{blue} 0.084 & \color{blue} 0.383 & \color{blue} 0.168\\
% }
5 & minhkhoi1026    & 0.00 & 0.004 & 0.226 & 0.034\\
\bottomrule
\end{tabular}
% } % \resizebox
\caption{
% 
Results in TextANIMAR \textit{test} set.
% 
} % \caption
\label{tab:sota}
\end{table*}
